Differential Privacy for Growing Databases

We study the design of differentially private algorithms for adaptive analysis of dynamically growing databases, where a database accumulates new data entries while the analysis is ongoing. We provide a collection of tools for machine learning and other types of data analysis that guarantee differential privacy and accuracy as the underlying databases grow arbitrarily large. We give both a general technique and a specific algorithm for adaptive analysis of dynamically growing databases. Our general technique is illustrated by two algorithms that schedule black box access to some algorithm that operates on a fixed database to generically transform private and accurate algorithms for static databases into private and accurate algorithms for dynamically growing databases. These results show that almost any private and accurate algorithm can be rerun at appropriate points of data growth with minimal loss of accuracy, even when data growth is unbounded. Our specific algorithm directly adapts the private multiplicative weights algorithm to the dynamic setting, maintaining the accuracy guarantee of the static setting through unbounded data growth. Along the way, we develop extensions of several other differentially private algorithms to the dynamic setting, which may be of independent interest for future work on the design of differentially private algorithms for growing databases.

==> instantiationsapp.tex <==
% !TEX root = main.tex
\section{ERM for Growing Databases}

\rc{I want to get rid of this appendix.  I moved B.1 into prelims.  We need to check that all relevant content from B.2 is covered in OldKevin}


\subsection{ERM Background}\label{ermapp}

Empirical risk minimization (ERM) is one of the most fundamental tasks in machine learning. In ERM, the task is to find a classifier from some set $\CC$ that minimizes a loss function $\LL$ on the sample data. Formally, we are given some data set $x_n = \{z_1,...,z_n\} \in \XX^n$, where each $z_i$ is sampled independently from some distribution $P$. We are also given some set $\CC$ such that for $\theta \in \CC$, the loss function $\LL$ is defined as:
\begin{align*}
\LL(\theta; x_n) = \frac{1}{n}\sum_{i=1}^n L(\theta; z_i)
\end{align*}
where for all $z\in \XX$, $L(\cdot;z)$ maps from $\CC$ to $\R$. Common choices for $L$ include the $0-1$ loss, hinge loss, and the squared loss. We seek to find a $\hat{\theta}$ with small \emph{excess empirical risk}, defined as
\begin{equation}\label{eq.risk}
\hat{\mathcal{R}}_n(\hat{\theta}) = \LL(\hat{\theta}; x_n) - \min_{\theta \in \CC} \LL(\theta; x_n)
\end{equation}
In convex ERM, we assume that $L(\cdot; x)$ is convex for all $x \in \XX$ and that $\CC$ is a convex set. We will also assume that $\XX\subseteq \R^p$. Convex ERM is convenient because finding a suitable $\hat{\theta}$ reduces to a convex optimization problem, for which there exist many fast algorithms. Some examples of ERM include finding a $d$-dimensional median and SVM.

ERM is useful due to its connections to the \emph{true risk}, also known as the generalization error, which we define as:
\begin{align*}
\mathcal{R}(\theta) = \E_{x \sim P}\br{L(\theta;x)}
\end{align*}
That is, the loss function will be low in expectation on a new data point sampled from $P$. We can also define the \emph{excess risk} of a classifier $\hat{\theta}$:
\begin{align*}
\textup{ExcessRisk}(\hat{\theta}) = \E_{x \sim P}\br{L(\hat{\theta};x)} - \min_{\theta \in \CC} \E_{x \sim P}\br{L(\theta;x)}
\end{align*}

ERM finds classifiers with low excess empirical risk, which in turn often have low excess risk. The following theorem relates the two. For completeness, we first give some definitions relating to convex empirical risk minimization sections. 
A convex body $\CC$ is a set such that for all $x,y\in \CC$ and all $\lambda \in [0,1]$, $\lambda x + (1-\lambda)y \in \CC$.	
 A vector $v$ is a subgradient of a function $L$ at $x_0$ if for all $x\in \CC$, $L(x) - L(x_0) \ge \langle v,x- x_0\rangle$.	
A function $L:\CC\ra \R$ is $G$-Lipschitz if for all pairs $x,y\in \CC$, $\abs{L(x) - L(y)} \le G\norme{x - y}$
 $L$ is $\Delta$-strongly convex on $\CC$ if for all $x \in \CC$ and all subgradients $z$ at $x$ and all $y \in \CC$, we have $L(y) \ge L(x) + \langle z, y - x\rangle + \frac{\Delta}{2} \norme{y - x}^2$.
$L$ is $B$-smooth on $\CC$ if for all $x\in \CC$, for all subgradients $z$ at $x$ and for all $y \in \CC$, we have $L(y) \le L(x) + \langle z, y- x\rangle + \frac{B}{2}\norme{y - x}^2$. 	
We denote the diameter of a convex set $\CC$ by $\norme{\CC} = \arg \max_{x,y\in \CC} \norme{x - y}$. 	


\begin{theorem}[\cite{shalev09}]
For $G$-Lipschitz and $\Delta$-strongly convex loss functions, with probability at least $1-\gamma$ over the randomness of sampling the data set $X_n$, the following holds:
\begin{align*}
\textup{ExcessRisk}(\hat{\theta}) \le \sqrt{\frac{2G^2}{\Delta}\hat{\mathcal{R}}_n(\hat{\theta})} + \frac{4G^2}{\gamma \Delta n}
\end{align*}     
\end{theorem}
Moreover, we can generalize this result to any convex and Lipschitz loss function $L$ by defining a regularized version of $L$, called $\tilde{L}$, such that $\tilde{L}(\theta; x) = L(\theta;x) + \frac{\Delta}{2}\norme{\theta}^2$. Then $\tilde{L}$ is $(L + \norme{\CC})$-Lipschitz and $\Delta$-strongly convex. Also note that:
\begin{align*}
\textup{ExcessRisk}_{L}(\theta) \le \textup{ExcessRisk}_{\tilde{L}}(\theta) +\frac{\Delta}{2}\norme{\CC}^2
\end{align*}
Thus, ERM finds classifiers with low true risk in these settings.

%\todo{find this paragraph a home} In the static setting, an algorithm for empirical risk minimization (ERM) takes in a database $x$ of size $n$, and outputs a classifier from some set $\CC$ that minimizes a loss function $\LL$ on the sample data.  Increasing the size of the training sample will improve accuracy of the classifier, as measured by excess empirical risk (Equation \eqref{eq.risk}).  Given the importance of ERM, it is no surprise that a number of previous works have considered differentially private ERM in the static setting \cite{CMS11, KST12, BST14}. 



%The growing ERM is as follows: 
\subsection{\ImprovingM{} for ERM} 

For ERM in the dynamic setting, we want a classifier $y_t$ at every time $t \geq n$ that achieves low empirical risk on the current database, and we want the empirical risk of our classifiers to improve over time, as in the static case.  Note that the dynamic variant of the problem is strictly harder because we must produce classifiers at every time step, rather than waiting for sufficiently many new samples to arrive.  Releasing classifiers at every time step degrades privacy, and thus requires more noise to be added to preserve the same overall privacy guarantee.  Nonetheless, we will compare our private growing algorithm, which provides accuracy bounds for every time step from $n$ to infinity simultaneously, to private static algorithms, which are only run once.  

%at every time step $t \ge n$, we want to have a classifier $y_t$ that achieves low empirical risk on the current database. However, we also want the empirical risk of our classifiers to improve over time, as in the static case. 

%If we didn't have to output classifiers at each time step, it would be best to wait until sufficiently many samples have arrived and then output a classifier. Releasing classifiers at every time step leaks privacy, so the growing problem is strictly harder. 



%Given the importance of ERM, it is no surprise that ERM has been considered in the context of DP. In this case, the sample $X_n$ forms the database, and a neighboring database differs in one sample. A number of previous works have given bounds for convex ERM \cite{CMS11, KST12, BST14}. 

In ERMG, our algorithm for ERM in the dynamic setting, the sole query of interest is the loss function $\LL$ evaluated on the current database.  At each time $t$, ERMG receives a single query $f_t$, where $f_t$ evaluated on the database is $x_t(f_t)=\min_{\theta\in\CC} \LL(\theta;x_t)$.  The black box  outputs $y_t$, which is a classifier from $\CC$ that can be used to evaluate the single query $y_t(f_t)=\LL(y_t;x_t)$.  Our accuracy guarantee at time $t$ is the difference between $y_t(f_t)$ and $x_t(f_t)$:
\begin{align*}
\alpha_t = \LL(y_t;x_t) - \min_{z\in\CC} \LL(z;x_t).
\end{align*}
This expression is identical to the excess empirical risk $\hat{\RR}_t(y_t)$ defined in Equation \eqref{eq.risk}.  Thus accurate answers to queries are equivalent to minimizing empirical risk. Our accuracy bounds are stated in \Cref{thm.erm}. The results come from instantiating (the more general) \Cref{thm.improvealpha}. The differing assumptions on $\LL$ allow us to use different ($p,g$)-black boxes with different input parameters in each case. We use the static $(\eps,0)$-DP algorithms of \cite{BST14} as black boxes.  We compare our growing bounds to these static bounds in \Cref{fig:erm}.\footnote{To get the static bounds, we use Appendix D of \cite{BST14}, which converts bounds on expected excess empirical risk to high probability bounds.} Since ERMG provides $(\eps,\delta)$-differential privacy, we also include static $(\eps,\delta)$-DP bounds from \cite{BST14, KST12} for comparison in \Cref{fig:erm}.  The static bounds are optimal in $d,t,$ and $\epsilon$ up to log factors. %The bounds we get are achieved using \ImprovingM{} and the accuracy bounds from \Cref{thm.improvealpha}.


\begin{restatable}{theorem}{ermthm}\label{thm.erm}
%\begin{theorem}\label{thm.erm}
Let $\LL$ be a convex loss function that is 1-Lipschitz over some set $\CC$ with $\norme{\CC} = 1$. Then for any stream of databases $X$ with points in $\mathbb{R}^d$, ERMG($X,\LL,\CC,\eps,\delta, \beta,n$) is $(\eps, \delta)$-differentially private and with probability at least $1-\beta$ produces classifiers $y_t$ for all $t \geq n$ that have excess empirical risk bounded by:
\begin{align*}
\hat{\RR}_t(y_t) \le \frac{d \sqrt{\log (1/\delta)}\log \frac{1}{\beta}}{\sqrt{c}\eps t^{\frac{1}{2} - c}}
\end{align*}
If $\LL$ is also $\Delta$-strongly convex,
\begin{align*}
\hat{\RR}_t(y_t) \le \frac{d^2 \log (1/\delta) \log^2 \frac{1}{\beta}}{\sqrt{c}\Delta \eps^2 t^{1-c}}
\end{align*}
where $c$ is any positive constant. 
%\end{theorem}
\end{restatable} 

\begin{proof}[Proof of Theorem~\ref{thm.erm}]
When the loss function is 1-Lipschitz and $\norme{\CC} = 1$, the $\epsilon$-differentially private static algorithm from \cite{BST14} is a $(p,g)$-black box for $p = 1$ and $g = d$. When the loss function is also $\Delta$-strongly convex, the $\epsilon$-differentially private static algorithm from \cite{BST14} is a $(p,p',p'',g)$-black box for $p = 2$, $p' = 2$, $p'' = 1$, and $g = d^2/\Delta$. %Finally, when the loss function is also $O(d)$-smooth (Case 3), the $\epsilon$-differentially private static algorithm from $\cite{CMS11}$ is a $(p,g)$-black box for $p = 2$ and $g = d^2/\Delta$.
The bounds of Theorem~\ref{thm.erm} come from instantiating \Cref{thm.improvealpha} using each of these black boxes.
%Then the bounds come directly from \Cref{thm.improvealpha}, where we also use the fact that for \Cref{thm.improvealpha}, the queries need not be normalized. 	
\end{proof}



%To clarify how we are comparing bounds, assume we have some data stream $\{D_t\}_{t=n}^\infty$. Then for the static algorithms, the bounds shown are the result of a static algorithm run on $D_t$ for some $t$. For the growing algorithm, we ensure the accuracy stated simultaneously for all $t$ from $n$ to $\infty$. \kl{redundant to state this twice?} 


%Then for all $t\in \{n,n+1,...\}$, we can use \ImprovingM{} to get a classifier $y_t$ such that the excess empirical risk $\hat{\RR}_t(y_t)$ is as follows:
%\begin{enumerate}
%	\item{With no further assumptions on $L$, \ImprovingM{} uses the $\epsilon$-DP algorithm of \cite{BST14} to get $\hat{\RR}_t(y_t) \le \frac{p \sqrt{\log (1/\delta)}\log \frac{1}{\beta}}{\sqrt{c}\eps t^{\frac{1}{2} - c}}$}
%	\item{If $L$ is also $\Delta$-strongly convex, \ImprovingM{} uses the $\epsilon$-DP algorithm of \cite{BST14} to get $\hat{\RR}_t(y_t) \le \frac{p^2 \log (1/\delta) \log^2 \frac{1}{\beta}}{\sqrt{c}\Delta \eps^2 t^{1-c}}$ }
%	\item{If $L$ is also $\Delta$-strongly convex and $O(p)$ smooth, \ImprovingM{} uses the $\epsilon$-DP algorithm of \cite{CMS11} to get $\hat{\RR}_t(y_t) \le \frac{p^2 \log (1/\delta) \log^2 \frac{1}{\beta}}{\sqrt{c}\Delta \eps^2 t^{1-c}}$ 
%		} 
%\end{enumerate}
%%where $c$ is any positive constant. Also, \ImprovingM{} is $(\eps,\delta)$-DP in all of these cases.

\renewcommand{\arraystretch}{1.75}
\begin{table}[h]
        \begin{tabular}{p{2.4cm} | c | c | c}
                Assumptions & Static $(\epsilon,0)$-DP & Static $(\epsilon,\delta)$-DP & Dynamic $(\epsilon,\delta)$-DP (our results) \\ \hline
                1-Lipschitz and $\mathcal {C} = 1$ & $\frac{d\log \frac{1}{\beta}}{\eps t}$  \cite{BST14} & $\frac{\sqrt{d} \log^2(t/\delta)\log \frac{1}{\beta}}{\eps t}$ \cite{BST14} & $\frac{d \sqrt{\log (1/\delta)}\log \frac{1}{\beta}}{\sqrt{c}\eps t^{\frac{1}{2} - c}}$ \\ \hline
                ... and $\Delta$-strongly convex (implies $\Delta \le 2$) & $\frac{d^2 (\log t)\log^2 \frac{1}{\beta}}{\Delta \eps^2 t^2}$ \cite{BST14} & $ \frac{d\log^3(t/\delta)\log^2 \frac{1}{\beta} }{\Delta  \epsilon^2 t^2}$ \cite{BST14} & $\frac{d^2 \log (1/\delta) \log^2 \frac{1}{\beta}}{\sqrt{c}\Delta \eps^2 t^{1-c}}$  
%\\ \hline                ... and $O(d)$-smooth & $\frac{d^2\log^2 \frac{1}{\beta}}{\Delta \eps^2 t^2}$ \cite{CMS11} & $\frac{d\log (1/\delta)\log^2 \frac{1}{\beta}}{\Delta \epsilon^2 t^2}$ \cite{KST12} & $\frac{d^2 \log (1/\delta) \log^2 \frac{1}{\beta}}{\sqrt{c}\Delta \eps^2 t^{1-c}}$
        \end{tabular}
        \caption{Comparison of excess empirical risk upper bounds in the static case versus the dynamic case for a database of size $t$ for different assumptions on the loss function $L$. Database entries are sampled from $\R^d$, and $c$ is any positive constant. We ignore leading multiplicative constants and factors of $\log \log \frac{1}{\beta}$ in the static bounds.  As in \cite{BST14}, we assume $\delta < 1/n$ for simplicity.\label{fig:erm} }
\end{table}


Note that the bounds we get for the growing setting have the same dependence on $\epsilon, \beta$, and $\Delta$ and better dependence on $\delta$. The dependence on $t$ in our bound is roughly the square root of that in the static bounds.  Compared to the static $(\epsilon,0)$-DP bounds, our dependence on $d$ is the same, while the dependence is squared relative to the static $(\epsilon,\delta)$-DP bounds.  

Given that the growing setting is strictly harder than the static setting, it is somewhat surprising that we have no loss in most of the parameters, and only minimal loss in the size of the database $t$. Thus, for ERM, performance in the static setting largely carries over to the growing setting.


